A Definition Of Quantum Mechanical Work

A definition of quantum mechanical work is introduced in this dissertation, preserving the mathematical structure of the Classical Mechanics concept of work without, however, in any way invoking the notion of trajectory. By use of Gaussian states and the Caldirola-Kanai model, a case study is conducted through which the proposed quantum work is compared with another Quantum Thermodynamics well-known definition, both in quantum and semiclassical regimes, showing promising results. Finally the new definition is investigated in comparison with a classical-statistical approach for superposition and mixed states.

==> resumo.tex <==
%\begin{center}
\chapter*{\normalsize \textbf{RESUMO}}
%\end{center}

\noindent A Mecânica Quântica pode ser vista como uma estrutura matemática que descreve resultados associados a sistemas microscópicos. Por outro lado, a Termodinâmica Clássica (juntamente com a Física Estatística) tem sido utilizada para caracterizar sistemas macroscópicos de forma geral, em que quantidades médias são consideradas e a conexão entre estas descrita de maneira formal por equações de estado. Com o intuito de relacionar essas teorias e desenvolver uma mais geral, trabalhos recentes têm sido desenvolvidos para conectar as ideias fundamentais da Termodinâmica com princípios quânticos. Este referencial teórico é ocasionalmente denominado Termodinâmica Quântica. Alguns conceitos chave associados a essa recente teoria são trabalho e calor, os quais estão bem estabelecidos no escopo da Termodinâmica Clássica e compõem a conservação de energia expressa pela primeira lei da Termodinâmica. Definições largamente aceitas para calor e trabalho foram introduzidas por Alicki em seu trabalho seminal de 1979. Embora, mostra-se, tais definições satisfaçam diretamente a primeira lei da Termodinâmica e têm sido aplicadas de forma bem sucedida a muitos contextos, parece não haver uma justificativa fundacional profunda para elas. De fato, definições alternativas foram propostas com base em analogias com a Termodinâmica Clássica. Na presente dissertação, uma definição de trabalho quântico-mecânico é introduzida, preservando a estrutura matemática do conceito clássico de trabalho sem, contudo, de forma alguma invocar a noção de trajetória. Com o uso de estados Gaussianos e do modelo de Caldirola-Kanai, um estudo de caso é conduzido através do qual o trabalho quântico ora proposto é comparado com a definição de Alicki, tanto em regime quântico como em semiclássico, mostrando resultados promissores. Inadequações conceituais são encontradas para o modelo de Alicki no limite clássico e possíveis interpretações são discutidas para a noção de trabalho quântico aqui introduzida. Finalmente, a nova definição é investigada em comparação com a abordagem clássico-estatística para estados de superposição e estados mistos. \\[1.5cm]  
\noindent \textbf{Palavras-chave:} Trabalho. Termodinâmica Quântica. Modelo de Caldirola-Kanai.



==> termoAprovacao.tex <==
%\begin{center}
\chapter*{TERMO DE APROVAÇÃO}
%\end{center}

Por meio deste termo, aprovamos a monografia do Projeto de Pesquisa "ANÁLISE TEÓRICO-NUMÉRICA DE MODELO CONSTITUTIVO PARA FLUIDOS TIXOTRÓPICOS", realizado pelo aluno Thales Augusto Barbosa Pinto Silva, como requisito para aprovação na disciplina Trabalho de Conclusão de Curso 2, do curso de Engenharia Mecânica da Universidade Tecnológica Federal do Paraná.
\vspace{2cm}
%
\bgroup
\def\arraystretch{1.5}% 
\begin{table}[h]
	\centering
	\begin{tabular}{lll}
		\cline{1-1} \cline{3-3}Prof. Ph.D Hilbeth Parente Azikri de Deus &  & Prof. Ph.D Cézar Otaviano Ribeiro Negrão \\
		Orientador & & Coorientador
	\end{tabular}
\end{table}

\vspace{2cm}
%\centering 
\begin{center}
	\textbf{Banca Examinadora}
\end{center}
\vspace{1.5cm}

\bgroup
\def\arraystretch{1.5}% 
\begin{table}[h]
	\centering
	\begin{tabular}{lll}                                 \cline{1-1} \cline{3-3}Prof. Dr. Admilson Teixeira Franco             &  & Prof. Dr. Silvio L. M. Junqueira      
	\end{tabular}
\end{table}

\pagebreak
